A New Defense Against Adversarial Images: Turning a Weakness into a Strength

Natural images are virtually surrounded by low-density misclassified regions that can be efficiently discovered by gradient-guided search --- enabling the generation of adversarial images. While many techniques for detecting these attacks have been proposed, they are easily bypassed when the adversary has full knowledge of the detection mechanism and adapts the attack strategy accordingly. In this paper, we adopt a novel perspective and regard the omnipresence of adversarial perturbations as a strength rather than a weakness. We postulate that if an image has been tampered with, these adversarial directions either become harder to find with gradient methods or have substantially higher density than for natural images. We develop a practical test for this signature characteristic to successfully detect adversarial attacks, achieving unprecedented accuracy under the white-box setting where the adversary is given full knowledge of our detection mechanism.

==> contents/related.tex <==
%!TEX root=main.tex
\section{Related Work}
\label{sec:related}
\WLC{not change yet}

Deep learning has become an increasingly important model in various tasks in computer vision. However, recent work by \cite{Szegedy2014} has shown that high dimensional data like image is very vulnerable to small perturbations. Several methods on adding perturbations on images has been proposed since then. Some of these methods are known as untargeted attacks where the algorithm generate adversarial images by optimizing a loss function to minimize the probability of the image to be the true class (\cite{Goodfellow2015}; \cite{Moosavi-Dezfooli2016}; \cite{Kurakin2017a};\cite{Xiao2018}). Other methods generate adversarial images are in a targeted setting where a label different from the true label is found and the algorithm optimizes a loss function to maximize the probability of the image to be that other label (\cite{Kurakin2017a}; \cite{Carlini2017a};\cite{Madry2018};). Both untargeted and targeted attack can build adversarial examples on images that fool the neural network.  

Several methods of increasing the model's robustness against adversarial examples have been proposed in earlier works. \cite{Goodfellow2015} first propose the idea of adversarial training where adversarial samples are included in the inputs of the neural network to train the network again. Later works by \cite{Kurakin2017b} used adversarial training on samples generated by FGSM which provides robustness to black-box attacks. \cite{Madry2018} did adversarial training with Projected Gradient Descent, providing robustness to the model in even white-box setting on MNIST and CIFAR. More recent works in adversarial training include \cite{Kanna2018} which embodied logit pairing loss and received significant improvement on ImageNet. 

Besides end-to-end adversarial training, a variety of methods have also been used to distinguish real and adversarial images. Feature-level differences between real and adversarial images \cite{Matzen2017} is examined but only on Resnet. Dimensionality reduction based defense \cite{Bhagoji2017} has shown Principal Component Analysis(PCA) can detect adversarial images on MNIST. Another class of detection method called distributional detect (\cite{Grosse2017};\cite{Feinman2017}).  Both methods works well on MNIST but poorly on CIFAR in either the black box \cite{Grosse2017} or the white box \cite{Feinman2017} setting. Image transformations has recently become a new trend of detecting adversarial examples. Adversarial samples are proven to be more vulnerable to some image transformations like total variation minimization and image quilting \cite{Guo2017}. Feature squeezing proposed by \cite{Xu2018} uses quantization and smoothing on black box attacks. \cite{Raghunathan2018} and \cite{Wong2018} has produced provable defense method proven theoretically on ReLU based simple fully connected neural networks.

